Local HI Absorption towards the Magellanic Cloud foreground using ASKAP

We present the largest Galactic neutral hydrogen HI absorption survey to date, utilizing the Australian SKA Pathfinder Telescope at an unprecedented spatial resolution of 30''. This survey, GASKAP-HI, unbiasedly targets 2,714 continuum background sources over 250 square degrees in the direction of the Magellanic Clouds, a significant increase compared to a total of 373 sources observed by previous Galactic absorption surveys across the entire Milky Way. We aim to investigate the physical properties of cold (CNM) and warm (WNM) neutral atomic gas in the Milky Way foreground, characterized by two prominent filaments at high Galactic latitudes (between $-45^{\circ}$ and $-25^{\circ}$). We detected strong HI absorption along 462 lines of sight above the 3$\sigma$ threshold, achieving an absorption detection rate of 17%. GASKAP-HI's unprecedented angular resolution allows for simultaneous absorption and emission measurements to sample almost the same gas clouds along a line of sight. A joint Gaussian decomposition is then applied to absorption-emission spectra to provide direct estimates of HI optical depths, temperatures, and column densities for the CNM and WNM components. The thermal properties of CNM components are consistent with those previously observed along a wide range of Solar neighborhood environments, indicating that cold HI properties are widely prevalent throughout the local interstellar medium. Across our region of interest, CNM accounts for ~30% of the total HI gas, with the CNM fraction increasing with column density toward the two filaments. Our analysis reveals an anti-correlation between CNM temperature and its optical depth, which implies that CNM with lower optical depth leads to a higher temperature.

==> 6_filaments.tex <==
\label{sec:filaments}
[THIS SECTION MAY BE NOT IMPORTANT]
In this section, we present an analysis of neutral atomic hydrogen gas toward HI filaments in the MC foreground. The HI filaments are defined as regions with high HI column density and high brightness temperature and are observed as the intersection of two distinct structures: vertical and horizontal, with lengths of 23 and 33 degrees, respectively, as shown in Figure \ref{fig:src_locations}. We here focus on investigating the variations of various HI quantities, such as column density, brightness temperature, and opacity correction factor, as a function of distance to these filaments. The aim of this analysis is to gain insights into the physical properties of HI gas in these structures by examining the trends and relationships between these quantities and distances. Figure \ref{fig:q_vs_distances} represents the distributions of the quantities with respect to the angular distances to the two filaments.

We find that the integrated properties of 528 sightlines with HI absorption detection, including \hi\ column density, maximum brightness temperatures, CNM cold gas fraction, HI opacity correction factors, and cold-warm \hi\ column density ratio ($f_\mathrm{c/w} = N_\mathrm{CNM}/N_\mathrm{WNM}$), exhibit a decreasing trend as moving away from the filaments. This is likely due to the decreasing gas density further from the filaments, which also leads to a decline in the amount of cold gas. Consequently, the warm-cold HI column density ratio ($f_\mathrm{w/c} = N_\mathrm{WNM}/N_\mathrm{CNM}$) varies from unity near the HI filaments to a value of $f_\mathrm{w/c} = 10$ at the furthest distance from the filaments.

==> 8_res_comparison.tex <==
In this section, we compare the results obtained by combining the GASKAP absorption dataset with high and low resolution emission datasets. Specifically, we perform the Gaussian decomposition using two different sets of data: (1) the GASKAP-only absorption+emission dataset, which has a high spatial resolution of 30 arcseconds, and (2) the GASKAP absorption dataset combined with the GASS emission dataset, which has a lower spatial resolution of 16 arcminutes.

The main purpose of this comparison is to investigate whether the GASKAP observation at high spatial resolution (30 arcseconds) would miss any details on the large-scale structure of the local Hi clouds. In particular, we are interested in understanding whether the use of a lower-resolution emission dataset could introduce any systematic biases in the derived Hi gas properties.

Our analysis reveals that the Hi gas properties obtained from the GASKAP and GASS emission datasets are consistent with each other. Specifically, we find that the Hi column densities and temperatures obtained from the two datasets are in good agreement, and that there is no significant difference in the distribution of Hi gas properties derived from the two datasets.

These results suggest that the GASKAP emission dataset at higher spatial resolution does not miss any extended large-scale structure of the Hi gas clouds in the high galactic latitudes. This is an important finding, as it confirms the validity of using the GASKAP dataset for studying the properties of the local Hi clouds, and provides a valuable baseline for future studies that use the GASKAP dataset in combination with other datasets.

==> AUTHORS.tex <==
\author[0000-0003-0742-2006]{Yik Ki Ma}
\affil{Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT~2611, Australia}

\author[0000-0002-5501-232X]{Antoine Marchal}
\affil{Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT~2611, Australia}


\author[0000-0003-2730-957X]{N.~M.\ McClure-Griffiths}
\affil{Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT~2611, Australia}


\author[0000-0002-7743-8129]{Claire E. Murray}
\affil{Space Telescope Science Institute, 
3700 San Martin Drive, 
Baltimore, MD, 21218}
\affil{Department of Physics \& Astronomy, 
Johns Hopkins University,
3400 N. Charles Street, 
Baltimore, MD 21218}


\author[0000-0002-9214-8613]{Helga D\'enes}
\affiliation{School of Physical Sciences and Nanotechnology, Yachay Tech University, Hacienda San Jos\'e S/N, 100119, Urcuqu\'i, Ecuador }


\author[0000-0002-6300-7459]{John M. Dickey}
\affiliation{School of Natural Sciences, Private Bag 37, University of Tasmania, Hobart, TAS, Australia}



\author[0000-0002-1495-760X]{Steven J. Gibson}
\affil{Department of Physics \& Astronomy, Western Kentucky University, 1906 College Heights Blvd., Bowling Green, KY 42101, USA}

\author[0000-0002-4814-958X]{Denis Leahy}
\affil{Department of Physics \& Astronomy, 
University of Calgary,
2500 University Dr. NW, 
Calgary, AB, Canada T2N 1N4}

\author[0000-0002-9888-0784]{Min-Young Lee}
\affil{Korea Astronomy and Space Science Institute, 
776 Daedeok-daero, Daejeon 34055, Republic of Korea}
\affil{Department of Astronomy and Space Science, 
University of Science and Technology, 
217 Gajeong-ro, Daejeon 34113, Republic of Korea}

\author[0000-0001-6846-5347]{Callum Lynn}
\affil{Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT~2611, Australia}


\author[0000-0002-2712-4156]{Hiep Nguyen}
\affil{Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT~2611, Australia}

\author[0000-0001-9504-7386]{Nickolas~M.~Pingel}
\affiliation{Department of Astronomy, The University of Wisconsin--Madison, 475 N. Charter Street, Madison, WI 53706, USA}


\author[0000-0002-1272-3017]{Jacco Th. van Loon}
\affil{Lennard-Jones Laboratories, Keele University, ST5 5BG, UK}

\author[0000-0002-1495-760X]{Steven J. Gibson}
\affil{Department of Physics \& Astronomy, Western Kentucky University, 1906 College Heights Blvd., Bowling Green, KY 42101, USA}

==> misc.tex <==
\subsection{Maths}
\label{sec:maths} % used for referring to this section from elsewhere

Simple mathematics can be inserted into the flow of the text e.g. $2\times3=6$
or $v=220$\,km\,s$^{-1}$, but more complicated expressions should be entered
as a numbered equation:

\begin{equation}
    x=\frac{-b\pm\sqrt{b^2-4ac}}{2a}.
	\label{eq:quadratic}
\end{equation}

Refer back to them as e.g. equation~(\ref{eq:quadratic}).

\subsection{Figures and tables}

Figures and tables should be placed at logical positions in the text. Don't
worry about the exact layout, which will be handled by the publishers.

Figures are referred to as e.g. Fig.~\ref{fig:example_figure}, and tables as
e.g. Table~\ref{tab:example_table}.

% Example figure
\begin{figure}
	% To include a figure from a file named example.*
	% Allowable file formats are eps or ps if compiling using latex
	% or pdf, png, jpg if compiling using pdflatex
	\includegraphics[width=\columnwidth]{example}
    \caption{This is an example figure. Captions appear below each figure.
	Give enough detail for the reader to understand what they're looking at,
	but leave detailed discussion to the main body of the text.}
    \label{fig:example_figure}
\end{figure}

% Example table
\begin{table}
	\centering
	\caption{This is an example table. Captions appear above each table.
	Remember to define the quantities, symbols and units used.}
	\label{tab:example_table}
	\begin{tabular}{lccr} % four columns, alignment for each
		\hline
		A & B & C & D\\
		\hline
		1 & 2 & 3 & 4\\
		2 & 4 & 6 & 8\\
		3 & 5 & 7 & 9\\
		\hline
	\end{tabular}
\end{table}
